On Approximability of Clustering Problems Without Candidate Centers

The k-means objective is arguably the most widely-used cost function for modeling clustering tasks in a metric space. In practice and historically, k-means is thought of in a continuous setting, namely where the centers can be located anywhere in the metric space. For example, the popular Lloyd's heuristic locates a center at the mean of each cluster. Despite persistent efforts on understanding the approximability of k-means, and other classic clustering problems such as k-median and k-minsum, our knowledge of the hardness of approximation factors of these problems remains quite poor. In this paper, we significantly improve upon the hardness of approximation factors known in the literature for these objectives. We show that if the input lies in a general metric space, it is NP-hard to approximate: $\bullet$ Continuous k-median to a factor of $2-o(1)$; this improves upon the previous inapproximability factor of 1.36 shown by Guha and Khuller (J. Algorithms '99). $\bullet$ Continuous k-means to a factor of $4- o(1)$; this improves upon the previous inapproximability factor of 2.10 shown by Guha and Khuller (J. Algorithms '99). $\bullet$ k-minsum to a factor of $1.415$; this improves upon the APX-hardness shown by Guruswami and Indyk (SODA '03). Our results shed new and perhaps counter-intuitive light on the differences between clustering problems in the continuous setting versus the discrete setting (where the candidate centers are given as part of the input).

==> cont.tex <==

\subsection{Conditional Inapproximability of Continuous \kmean and \kmed}\label{sec:condCont}

\iffalse %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this subsection, we show how \JCH implies the hardness of approximation of Euclidean \kmean and $\ell_1$-metric \kmed, both in the continuous case and i.e., we prove Theorems~\ref{thm:introell2without}~and~\ref{thm:introell1without}.

In order to prove the results in this section, we need to assume a slight strengthening of \JCH. 
\begin{hypothesis}[Dense Johnson Coverage Hypothesis (\JCHD)]
\JCH holds for instances $(U,E,k)$ of Johnson coverage problem where $|E|=\omega(k)$.
\end{hypothesis}

Even in \cite{CK19}, where the authors proved the previous best inapproximability results for continuous case \kmean and \kmed, they needed a similar condition. In their case, they were reducing from $(0.9292,2)$-Johnson coverage problem (whose hardness was known under unique games conjecture \cite{AS19}) and it was easy to show that the hard instances had this additional property by opening up the reduction in \cite{AS19} (actually this part was shown in prior work of \cite{AKS11}). 

Nonetheless, the additional  property that we desire, while fairly reasonable, has always been obtained in literature by looking at the hard instances that were constructed. It would be interesting to prove that the hard instances have this additional property in a blackbox manner, i.e., we would like to show that \JCH implies \JCHD. We make some progress on this problem in the below lemma and note that it even simplifies part of the proof of \cite{AKS11}. 

\begin{lemma}\label{lem:JC}
Let $\alpha\in [0,1]$ and $z\in\mathbb N$. Given an instance $(U,E,k)$ of $(\alpha,2)$-Johnson coverage problem, there is a polynomial time (in $|U|$ and $|E|$) reduction to an instance $(U',E',k')$ of $(\alpha,2)$-Johnson coverage problem such that the following holds:
\begin{itemize}
\item $(U,E,k)$ is a YES instance if and only if $(U',E',k')$ is a YES instance, and
\item  $|E'|=\omega(k')$. 
\end{itemize} 
\end{lemma}
\begin{proof}

\end{proof}


We return to showing the main results of this subsection. First, we consider Euclidean \kmean. 
\fi %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this subsection, we show how \JCH implies the hardness of approximation of Euclidean \kmean and $\ell_1$-metric \kmed, both in the continuous case and i.e., we prove Theorem~\ref{thm:introell2without}.
In order to prove the results in this section, we need to assume a slight strengthening of \JCH. 
\begin{hypothesis}[Dense Johnson Coverage Hypothesis (\JCHD)]
\JCH holds for instances $(U,E,k)$ of Johnson coverage problem where $|E|=\omega(k)$.
\end{hypothesis}

This additional property has always been obtained in literature by looking at the hard instances that were constructed. 
In \cite{CK19}, where the authors proved the previous best inapproximability results for continuous case \kmean and \kmed, 
it was observed that hard instances of $(0.9292,2)$-Johnson Coverage constructed in~\cite{AKS11, AS19} can be made to satisfy the above property.

First, we consider Euclidean \kmean.  

\begin{theorem}[\kmean without candidate centers in $O(\log n)$ dimensional Euclidean space]\label{thm:kmeanl2}
Assuming \JCHD, for every constant $\varepsilon>0$,  given a point-set $\Po\subset \{0,1\}^{d}$ of size $n$ (and $d=O(\log n)$) and a parameter $k$ as input, it is \NP-hard to distinguish between the following two cases:
\begin{itemize}
\item \textbf{\emph{Completeness}}:  
There exists $\C':=\{c_1,\ldots ,c_k\}\subseteq \mathbb R^d$ and $\sigma:\Po\to\C'$ such that $$\sum_{a\in\Po}\|a-\sigma(a)\|_2^2\le \rho n\log n,$$
\item \textbf{\emph{Soundness}}: For every $\C':=\{c_1,\ldots ,c_k\}\subseteq \C$ and every $\sigma:\Po\to\C'$ we have: $$\sum_{a\in\Po}\|a-\sigma(a)\|_2^2\ge \left(1+\frac{1}{e}-\varepsilon\right)\cdot \rho n\log n,$$
\end{itemize}
for some constant $\rho>0$.
\end{theorem}
\begin{proof}
The construction of the point-set $\Po$ in the theorem statement is the same as in the proof of Theorem~\ref{thm:kmeanellp} (with a further simplification as we fix the embedding given in Lemma~\ref{lem:cd2}). However, the soundness analysis to prove the theorem is more intricate. 

Fix $\varepsilon>0$ as in the theorem statement. Also, fix $p\in\met$. Let $\eps':=\eps/11$. Starting from a hard instance of $\left( 1-\frac{1}{e}+\eps',z:=z(\eps')\right)$-Johnson coverage problem $(U,E,k)$  guaranteed by  \JCHD (i.e., $|E|=\omega(k)$),
  we create an instance of the \kmean using  Algebraic-Geometric codes and the embedding given in Lemma~\ref{lem:cd2}  as follows. Let $q$ be a (constant) prime square greater than $\left(\frac{18z^2}{\eps'}\right)^2$. Let $\AG$ be the code guaranteed by Theorem~\ref{thm:code}  over alphabet of size $q$ of message length $\eta:=\log_q n$ (recall $|U|=n$), block length $\ell:=O_{q}(\eta)$, and relative distance at least $1-\nicefrac{3}{\sqrt{q}}$. 
  

\paragraph{Construction.}  The  \kmean instance consists of the set of points to be clustered $\Po\subseteq \{0,1\}^{\ell\cdot q}$ which will be defined below. 
 Recall the function $A_E:E\times [\ell]\to \binom{[q]}{z}\cup \{\perp\}$ defined in the proof of Theorem~\ref{thm:kmeanellp} (also recall the definitions  $R_{T,\gamma}^{z}$, $\Lambda_{x,y}$, $L_T^{z},\tilde A_F$). We construct $\tilde A_E:E\to\{0,1\}^{q\cdot \ell}$ below.  Given $\tilde A_E$ the point-set $\Po$ is just defined to be $$\left\{\tilde A_E(T)\big| T\in E\right\}.$$

Let $\tau$ map a subset of $[q]$ to its characteristic vector in $\{0,1\}^q$. Now we can construct $\tilde A_E$ as follows:
$$\forall \gamma\in[\ell], \ 
\tilde A_E(T)\lvert_{\gamma}=\begin{cases} \tau(A_E(T,\gamma)) \text{ if } A_E(T,\gamma)\neq \perp\\ \tau(\Lambda_{|R_{T,\gamma}^z|,z}(R_{T,\gamma}^{z}))\text{ otherwise}\end{cases}.$$


\paragraph{Structural Observations.}
We  compute distances in a couple of cases.   
Consider  distinct $T,T'\in E$ such that $|T\cap T'|=z-1$. Then we have
\begin{align}\label{eqsub}
(2-\delta)\cdot{\ell}\le \|\tilde{A}_E(T)-\tilde{A}_E(T')\|_2^2\le {2\ell}
,\end{align}
where $\delta:= 18z^2/\sqrt{q}$ (note that $\delta\le \eps'$).
%To see this, first let $T\cap T':=S\in\binom{[n]}{z-1}$, $T\setminus T':=\{u_T\}$, and $T'\setminus T:=\{u_{T'}\}$. 
% This is because, if $S\subset T$ then for all $\gamma\in[\ell]$ we have $R_{S,\gamma}^{z-1}\subseteq R_{T,\gamma}^z$. Fix $\gamma\in [\ell]$. If $\gamma\in L_{S,T}$ then we have that $ \|\tilde{A}_E(T)|_\gamma-\tilde{A}_F(S)|_\gamma\|_p^p=\beta^p$ as $(R_{S,\gamma}^{z-1},R_{T,\gamma}^z)$ is an edge in $J(q,z)$. On the other hand if $\gamma\notin L_{T}^z$ then either $\gamma\notin L_{S}^{z-1}$ and we have that $\Lambda_{|R_{S,\gamma}^{z-1}|,z-1}(R_{S,\gamma}^{z-1})\subseteq \Lambda_{|R_{T,\gamma}^z|,z}(R_{T,\gamma}^z)$ because $R_{S,\gamma}^{z-1}\subseteq R_{T,\gamma}^z$, or we have $\gamma\in L_{S}^{z-1}$, in which case, we have $R_{T,\gamma}^z=R_{S,\gamma}^{z-1}$ and thus $R_{S,\gamma}^{z-1}\subseteq \Lambda_{|R_{T,\gamma}^z|,z}(R_{T,\gamma}^z)$. In the former case, we have that $(\Lambda_{|R_{S,\gamma}^{z-1}|,z-1}(R_{S,\gamma}^{z-1}),\Lambda_{|R_{T,\gamma}^z|,z}(R_{T,\gamma}^z))$ is an edge in $J(q,z)$ and in the latter case we have that $(R_{S,\gamma}^{z-1},\Lambda_{|R_{T,\gamma}^z|,z}(R_{T,\gamma}^z))$ is an edge in $J(q,z)$. The final result in both cases is that $ \|\tilde{A}_E(T)|_\gamma-\tilde{A}_F(S)|_\gamma\|_p^p=\beta^p$. Therefore, we have  $$\sum_{\gamma\in[\ell]}\|\tilde{A}_E(T)|_\gamma-\tilde{A}_F(S)|_\gamma\|_p^p=\|\tilde{A}_E(T)-\tilde{A}_F(S)\|_p^p=\beta^p\cdot \ell.$$

Now consider  distinct $T,T'\in E$ such that $|T\cap T'|<z-1$. Then we have 
\begin{align}\label{eqnosub}
(4-\delta)\cdot{\ell}\le \|\tilde{A}_E(T)-\tilde{A}_E(T')\|_2^2.
\end{align}
%Let $u\in U$ such that $u\in S$ but $u\notin T$. We define $\Good:=\{\gamma\in[\ell]: \AG(u)_\gamma\notin R_{T,\gamma}^z\}$. Since the relative distance of $\AG$ is $1-\nicefrac{3}{\sqrt{q}}$, we have by simple union bound that $$|\Good|\ge \left(1-\frac{3z}{\sqrt{q}}\right)\cdot\ell.$$  
% To see this first observe that $$\|\tilde{A}_E(T)-\tilde{A}_F(S)\|_p^p\ge \sum_{\gamma\in L_{S,T}\cap \Good}\|\tilde{A}_E(T)|_\gamma-\tilde{A}_F(S)|_\gamma\|_p^p.$$ 
%Fix $\gamma\in L_{S,T}\cap \Good$. Notice that $R_{S,\gamma}^{z-1}\not\subset R_{T,\gamma}^z$ and thus $(R_{S,\gamma}^{z-1},R_{T,\gamma}^z)$ is not an edge in $J(q,z)$. Therefore, we have
%$$\|\tilde{A}_E(T)|_\gamma-\tilde{A}_F(S)|_\gamma\|_p^p\ge g_p(J(q,z))^p\cdot \beta^p.$$ 
%Since $|L_{S,T}\cap \Good|\ge \left(1-\nicefrac{3z}{\sqrt{q}}-\nicefrac{3z(z-1)}{\sqrt{q}}\right)\cdot \ell\ge \left(1-\nicefrac{6z(z-1)}{\sqrt{q}}\right)\cdot \ell$, \eqref{eqbad} follows immediately by noting that (i) $g_p(J(q,z))\le 3$, and (ii) for any $\eta\in[0,1]$, $(1-\eta)^{1/p}\ge (1-\eta)$.
  
We now analyze the \kmean  cost of the
instance.
To do so, we will make use of the following classic fact about the $k$-means cost of a partition $C_1\dot\cup\cdots\dot\cup C_k=\Po$ of a set of
points in $\R^d$.
\begin{fact}
  \label{fact:kmeanscost}
  Given a clustering $C_1\dot\cup\cdots\dot\cup C_k=\Po$, the \kmean cost
  is exactly
  $$\sum_{i=1}^k \frac{1}{2|C_i|} \sum_{p \in C_i} \sum_{q \in C_i} \|p-q\|^2_2.
  $$
\end{fact}


Consider the completeness case first. 
\paragraph*{Completeness.}
  Suppose there exist $S_1,\ldots ,S_k\in \binom{[n]}{z-1}$ such that $\underset{i\in[k]}{\bigcup}\con(S_i,E)=E$. Then, we define a clustering $C_1\dot\cup\cdots\dot\cup C_k=\Po$  as follows: for every $a\in\Po$, where $a:=\tilde A_E(T)$ for some $T\in E$, let $a\in C_i$  such that $T\in \con(S_i,E)$ (if there is more than one $i\in[k]$ for which $S_i$ is contained in $T$ then we choose one arbitrarily).
We now provide an upper bound on the $k$-means cost of clustering $\mathcal{C}:=\{C_1,\ldots ,C_k\}$.
Equation~\ref{eqsub} implies that for each $C_i$, for any pair $T, T'$ such that
$\tA_E(T), \tA_E(T') \in C_i$, we have that $||\tA_E(T) - \tA_E(T') ||^2_2 \le 2\ell$.
Hence,
$$\frac{1}{2|C_i|} \sum_{q \in C_i} \sum_{p \in C_i} ||p-q||^2_2 \le
\frac{1}{2|C_i|} \sum_{q \in C_i} \sum_{p \in C_i, p \neq q} 2\ell\le 
(|C_i|-1) \ell.
$$
Thus, the cost of clustering $\C$ is at most
$\ell (|\Po|-k)$.
Finally, we turn to the soundness analysis.

\paragraph*{Soundness.}
Consider the optimal $k$-means clustering $\mathcal{C}:=\{C_1,\ldots ,C_k\}$  of the instance (i.e., $C_1\dot\cup\cdots\dot\cup C_k=\Po$). We aim at showing that the $k$-means cost of $\C$ is at
least $(1+1/e-\eps)\ell (|\Po|-k)$. Given a cluster $C_i$, for each
$S \in {[n] \choose z-1}$, we define the \emph{degree of $S$ in $C_i$}
to be $$d_{S,i} := 
\left|\{T \mid S \subset T \text{ and } \tA_E(T) \in C_i\}\right|.$$
The soundness analysis relies on the following claim.
\begin{claim}
  \label{claim:sumdegsquared}
  For every $i\in[k]$ we define 
  $$
  \Delta_i=\underset{S\in\binom{[n]}{z-1} }{\max}\ d_{S,i}.
  $$
  For every $\alpha\in (0,\nicefrac{1}{2})$ and
  cluster $C_i$ such that $|C_i| \ge 10/\alpha^{10}$,
we have  $$\cost(C_i) \ge (2-\delta/2)|C_i| \ell - (1+(z+O(1))\alpha)\Delta_i\ell.$$\end{claim}

%% We claim that the contribution to
%% the cost by the points of the cluster is at least
%% $2|C_i| +2 - \Delta_i$.
Assume Claim~\ref{claim:sumdegsquared} is true for a moment
and let's complete the proof of the soundness case.
We apply Claim~\ref{claim:sumdegsquared} with $\alpha = \eps_0/z$.
Then, observe that since the number of clusters is
$k < 10 z^{10} |E|/\eps^{11}_0$
then by averaging the total
number of elements $T$ such that $\tA_E(T)$ is in a cluster $C_i$
such that $|C_i| < 10(z/\eps_0)^{10}$
is at most $\eps_0 |E|$.
Thus, let's simply bound the cost for the elements in clusters of size
at least
$10(z/\eps_0)^{10}$. Let $k'$ be the number of such clusters.
Summing up over all such clusters, we have that the total $k$-means
cost is at least
$\ell\sum_{i=1}^{k'} (2-\delta/2)|C_i|-(1+O(\eps_0))
\Delta_i \ge (2-\delta/2)|E|\ell
- (1+O(\eps))\ell\sum_{i=1}^{k'} \Delta_i$, since $\eps \le 1/2$.
Then, to provide a lower bound on $\Delta_i$, consider
the set $\C = \{S_1,\ldots,S_k\}$. This set has size at most
$k$ and so by definition of the soundness
case we have $\con(\C) \le (1-1/e+\eps)|E|$ and therefore
$(1+O(\eps))\ell\sum_{i=1}^{k'} \Delta_i \le (1-1/e+O(\eps))|E|\ell$.
It follows that the cost of the optimal solution is at least
$(1+1/e-\delta/2-O(\eps))\ell$ as claimed.


We can thus conclude the proof of the above theorem by proving Claim~\ref{claim:sumdegsquared}.
\begin{proof}[Proof of Claim~\ref{claim:sumdegsquared}]
  Consider a cluster $C_i$ such that $|C_i| \ge 10/\eps^{3z}$. Let
  $E_i = \{T \in E \mid \tA_E(T) \in C_i\}$. Fix an arbitary ordering $\sigma$ of the elements of the universe.
  Consider an element $T \in E_i$. For each $1 \le j \le z$, we let
  $T^j$ be the element of ${n \choose z-1}$ obtained by removing the $i$th element of $T$, in the order $\sigma$.
  Then, let $\Sigma_T = -t + \sum_{j=1}^z d_{i, T^j}$.
  
  By Equations~\ref{eqbad},~\ref{eqsub}
  we have that 
  \begin{align*} \frac{1}{2|C_i|} \sum_{T' \in E_i} \|\tA_E(T)-\tA_E(T')\|^2_2 
  &\ge
  \frac{\ell}{2|C_i|} \left((2-\delta) \Sigma_T + (4-\delta)(|C_i|-\Sigma_T)\right)\\
  &\ge \frac{\ell}{|C_i|} ((2-\delta/2)|C_i|-\Sigma_T)\\
  &\ge (2-\delta/2)\ell - \frac{\ell\Sigma_T}{|C_i|}.
  \end{align*}
%% $C_i$ and which are adjacent to $u_i$ or $u_j$.
%% This is thus
%% $$\frac{1}{2|C_i|} \left(2(|C_i|-1) + 2(|C_i|-d_{i,\ell} - d_{i,j} + 2\right).$$
  Now, summing up over all $T$ in $E_i$ gives a total cost for the cluster $C_i$
  of at least
  \[ |C_i|(2-\delta/2)\ell - \frac{\ell}{|C_i|} \sum_{T\in E_i} \Sigma_T \ge
  |C_i|(2-\delta/2)\ell - \frac{\ell}{|C_i|} \sum_{S\in {n \choose z-1}} d_{i,S}^2. \]
  The rest of the proof consists in providing an upper bound on $\sum_{S\in {n \choose z-1}} d_{i,S}$.


  
  First, consider the set $\S = \{S \in {n\choose z-1} \mid d_{i,S} < \eps |C_i|\}$,
  and let $E^0_i = \{T \in E_i \mid \exists S \in \S, S \subseteq T\}$
  We have that
  \begin{equation}
    \label{eq:lowdegrees}
    \frac{1}{|C_i|} \sum_{S \in \S} d^2_{i,S} \le \frac{\eps |C_i|}{|C_i|} \sum_{S \in \S} d_{i,S} \le
    2 \eps |E^0_i|.
  \end{equation}
  
  We then bound $\sum_{S \notin \S} d^2_{i,S}$.
  Let $\S' = {n \choose z-1} \setminus \S$
  and $E^1_i = \{T \in E_i \mid \exists S_1,S_2 \in \S', S_1 \neq S_2, S_1 \subseteq T, S_2 \subseteq T\}$.
  We claim that
  \begin{equation}
    \label{eq:sumofdegrees}
    \sum_{S \in \S'} d_{i,S} \le (z-1)|E_i^1|+|E_i|.
  \end{equation}
  Indeed, consider an element $T \in E_i$, we have that either there is at most one element $S$ of $\S'$ such that
  $S \subset T$, in which case $T$ will be counted at most once in $\sum_{S \in \S'} d_{i,S}$, or
  $T$ contains more than one element of $\S'$. In the latter case we have that since
  each $S \in \S'$ is a $z-1$-tuple and each $T \in E_i$ is a $z$-tuple, we have that $T$ can contribute to
  the degree $d_{i,S}$ of at most $z$ different sets.
  Therefore, the elements of $E^1_i$ are counted at most $z$ times in the sum and from there follows
  Equation~\ref{eq:sumofdegrees}.

  
  We then prove that $|E^1_i| < \eps |E_i|$.  From Equation~\ref{eq:sumofdegrees} we deduce that
  there exists $S \in \S'$ such that $d_{i,S} \le (E^1_i + |E_i|)/|\S'|$. Moreover, since $S \in \S'$ we also
  have that $d_{i,S} \ge \eps|E_i| \ge \eps|E^1_i|$ and so, combining the two bounds yields
  $\eps|E^1_i| \le (E^1_i + |E_i|)/|\S'|$.
  Rearranging gives
  \[
  |\S'| \le 1/\eps + \frac{|E_i|}{\eps|E^1_i|}.
  \]
  Now, assuming toward contradiction $|E^1_i| > \eps|E_i|$ we get $|\S'| \le (1+\eps)/\eps^2 $. Hence,
  $|E^1_i| $ is at most $((1+\eps)/\eps^2)^2$ since for each pair $S,S' \in \S'$, $S \neq S'$ there is at most one
  $T \in E_i$ such that $S \subset T, S' \subset T$.
  Thus, $|C_i| = |E_i| \le ((1+\eps)/\eps^2)^4$, a contradiction to our assumption on $C_i$.
  Therefore $|E^1_i| \le \eps |E_i|$.
  
  We can now bound  $\sum_{S \notin \S} d^2_{i,S}$.
  Using Eq~\ref{eq:sumofdegrees} together with the above bound on $|E^1_i|$, we obtain
  \begin{equation}
    \label{eq:largedegrees}
    \sum_{S \notin \S} d^2_{i,S} \le \Delta_i \sum_{S \notin \S} d_{i,S} \le \Delta_i (|E_i| + (z-1)|E^1_i|) \le
    \Delta_i (1+(z+O(1))\eps)|E_i|.
  \end{equation}  
  
  Finally, combining Equations~\ref{eq:lowdegrees} and~\ref{eq:largedegrees} we deduce that
  $\frac{1}{|E_i|}\sum_{S} d^2_{i,S} \le  (1+(z+O(1))\eps)\Delta_i$.
  Therefore, recalling $|E_i| = |C_i|$,
  the cost of cluster $C_i$ is at least 
  $ (2-\delta/2)|C_i| \ell - (1+(z+O(1))\eps)\Delta_i \ell$.
\end{proof}



    
    
\end{proof}


Before, we address continuous case of \kmed in $\ell_1$-metric, we prove hardness of approximating the continuous case of both \kmean and 
\kmed in the Hamming metric. The inapproximability of \kmed in $\ell_1$-metric then follows by a simple observation. 

\begin{theorem}[\kmed without candidate centers in $O(\log n)$ dimensional $\ell_0$-metric space]\label{thm:kmedHam}
Assuming \JCHD, for every constant $\varepsilon>0$,  given a point-set $\Po\subset \{0,1\}^{d}$ of size $n$ (and $d=O(\log n)$) and a parameter $k$ as input, it is \NP-hard to distinguish between the following two cases:
\begin{itemize}
\item \textbf{\emph{Completeness}}:  
There exists $\C':=\{c_1,\ldots ,c_k\}\subseteq \mathbb \{0,1\}^d$ and $\sigma:\Po\to\C'$ such that $$\sum_{a\in\Po}\|a-\sigma(a)\|_0\le \rho n\log n,$$
\item \textbf{\emph{Soundness}}: For every $\C':=\{c_1,\ldots ,c_k\}\subseteq \{0,1\}^d$ and every $\sigma:\Po\to\C'$ we have: $$\sum_{a\in\Po}\|a-\sigma(a)\|_0\ge \left(1+\frac{1}{e}-\varepsilon\right)\cdot \rho n\log n,$$
\end{itemize}
for some constant $\rho>0$.
\end{theorem}


\begin{theorem}[\kmean without candidate centers in $O(\log n)$ dimensional $\ell_0$-metric space]\label{thm:kmeanHam}
Assuming \JCHD, for every constant $\varepsilon>0$,  given a point-set $\Po\subset \{0,1\}^{d}$ of size $n$ (and $d=O(\log n)$) and a parameter $k$ as input, it is \NP-hard to distinguish between the following two cases:
\begin{itemize}
\item \textbf{\emph{Completeness}}:  
There exists $\C':=\{c_1,\ldots ,c_k\}\subseteq \mathbb \{0,1\}^d$ and $\sigma:\Po\to\C'$ such that $$\sum_{a\in\Po}\|a-\sigma(a)\|_0^2\le \rho n(\log n)^2,$$
\item \textbf{\emph{Soundness}}: For every $\C':=\{c_1,\ldots ,c_k\}\subseteq \{0,1\}^d$ and every $\sigma:\Po\to\C'$ we have: $$\sum_{a\in\Po}\|a-\sigma(a)\|_0^2\ge \left(1+\frac{3}{e}-\varepsilon\right)\cdot \rho n(\log n)^2,$$
\end{itemize}
for some constant $\rho>0$.
\end{theorem}

\begin{proof}[Proof of Theorems \ref{thm:kmedHam} and \ref{thm:kmeanHam}]
The construction of the point-set $\Po$ in the theorem statement is the same as in the proof of Theorem~\ref{thm:kmeanl2}. 
 The completeness case is the same as in Theorem~\ref{thm:kmeanellp}. Therefore, we have that  the \kmean cost of the overall instance is at most $ \ell^{2}\cdot |\Po|$, while the \kmed cost is at most
  $\ell\cdot|\Po|$. 
The soundness analysis to prove the theorem follows by a case analysis, which is elaborated in \cite{CK19} and we skip it here for the sake of brevity.  
\end{proof}

Finally, we consider below \kmed in $\ell_1$-metric. 

\begin{theorem}[\kmed without candidate centers in $O(\log n)$ dimensional $\ell_1$-metric space]\label{thm:kmedl1}
Assuming \JCHD, for every constant $\varepsilon>0$,  given a point-set $\Po\subset \{0,1\}^{d}$ of size $n$ (and $d=O(\log n)$) and a parameter $k$ as input, it is \NP-hard to distinguish between the following two cases:
\begin{itemize}
\item \textbf{\emph{Completeness}}:  
There exists $\C':=\{c_1,\ldots ,c_k\}\subseteq \mathbb \R^d$ and $\sigma:\Po\to\C'$ such that $$\sum_{a\in\Po}\|a-\sigma(a)\|_1\le \rho n\log n,$$
\item \textbf{\emph{Soundness}}: For every $\C':=\{c_1,\ldots ,c_k\}\subseteq \R^d$ and every $\sigma:\Po\to\C'$ we have: $$\sum_{a\in\Po}\|a-\sigma(a)\|_1\ge \left(1+\frac{1}{e}-\varepsilon\right)\cdot \rho n\log n,$$
\end{itemize}
for some constant $\rho>0$.
\end{theorem}
\begin{proof}[Proof Sketch]
  The proof follows from a simple observation that for instances where all
  the coordinates of the points to be clustered are in $\{0,1\}$, we have
that for any subset (i.e. cluster) of the points of the instance,
  an optimal center of the set is such that its 
  $i$th coordinate is the median
  of a set of values in $\{0,1\}$, i.e., we may assume without loss of generality that the $i$th coordinate of the center is also in $\{0,1\}$. Therefore, simply  mimicking
  the proof of Theorem~\ref{thm:kmedHam} yields the desired theorem statement.
See \cite{CK19} for a formal argument.   
  \end{proof}

%\enote{Should be able to make $O(\log n$)-dim. Just I am not comfortable enough to write this..}

Finally, we finish the section by proving the remaining hardness results for continuous \kmed and \kmean:
\kmed in $\ell_2$-metric and 
\kmean in $\ell_1$-metric.
Especially, \kmed in $\ell_2$-metric for $k = 1$ is known as the {\em geometric median} and is  actively studied for bounded $d$ or $k$~\cite{arora1998approximation, badoiu2002approximate, kumar2010linear, feldman2011unified}, but to the best of our knowledge, no (hardness of) approximation algorithms have been studied for general $d$ and $k$. 
First, we prove the following lemma.

\begin{lemma}\label{lem:hypergraph_l2}
Let $H = (V, E)$ be an $r$-uniform $(r \geq 1)$ hypergraph where each vertex belongs to least one hyperedge, and $x : V \to [0, 0.5]$ such that
\begin{equation*}
y(e) := \sum_{v \in e} (1 - x_v)^2 + 
\sum_{v \in E \setminus e} x_v^2 \leq 1 + 0.25(r - 1) - \eps \quad \forall e \in E. 
\end{equation*}
for some $\eps > 0$. Then $|E| \leq (8r / \eps^2 + r)^r$. 
\end{lemma}
\begin{proof}
Suppose that every $v$ satisfies $x_v \geq \sqrt{2r / (n - r)}$. Then for any $e \in E$, 
\[
y(e) \geq \sum_{v \in E \setminus e} x_v^2 \geq (n-r) \frac{2r}{n-r} = 2r,
\]
leading to contradiction. Therefore, there is $v \in V $ that satisfies 
$x_v < \sqrt{2r / (n - r)}$. Choose a hyperedge $e$ containing $v$. Then 
\begin{align*}
& 1 - \eps + 0.25(r - 1) \geq y(e) \geq (1 - x_v)^2 + \sum_{u \in e \setminus \{ v \}} x_u^2 \geq 1 - 2x_v + 0.25(r - 1) \\ \geq & 1 - 2\sqrt{\frac{2r}{(n - r)}} + 0.25(r-1),
\end{align*}
which implies 
\[
\eps \leq 2\sqrt{\frac{2r}{(n - r)}} \Leftrightarrow n \leq \frac{8r}{\eps^2} + r
\]
The lemma follows by noting that $|E| \leq n^r$. 
\end{proof}

\begin{theorem}[\kmed without candidate centers in $O(\log n)$-dimensional $\ell_2$-metric space]\label{thm:kmedl2}
Assuming \JCHD, for every constant $\varepsilon>0$,  given a point-set $\Po\subset \{0,1\}^{d}$ of size $n$ (and $d=O(\log n)$) and a parameter $k$ as input, it is \NP-hard to distinguish between the following two cases: 
\begin{itemize}
\item \textbf{\emph{Completeness}}:  
There exists $\C':=\{c_1,\ldots ,c_k\}\subseteq \mathbb \R^d$ and $\sigma:\Po\to\C'$ such that $$\sum_{a\in\Po}\|a-\sigma(a)\|_2\le n$$
\item \textbf{\emph{Soundness}}: For every $\C':=\{c_1,\ldots ,c_k\}\subseteq \R^d$ and every $\sigma:\Po\to\C'$ we have: $$\sum_{a\in\Po}\|a-\sigma(a)\|_2\ge \left(1-1/e+\frac{\sqrt{1.25}}{e}-\varepsilon\right)n \approx 1.0434n.$$
\end{itemize}
%for some constant $\rho>0$.
\end{theorem}
\begin{proof} 
Given an instance $(U, E, k)$ of $(1-1/e+\eps, z)$-\jc for small fixed $\eps > 0$, for any $S \subseteq U$, let $\tau(S)$ be the indicator vector of $S$. (The dimension can be reduced to $O(\log n)$ by the standard dimension reduction technique.) 

In the completeness case, every point is connected to a center at distance $1$.
For the soundness case, fix one cluster $C$ and its center $c \in \R^U$.
Fix $\eps > 0$, and remove all points from $C$ whose $\ell_2^2$ distance to $c$ is greater than $(1.25 - \eps)$.
Assume $C = \omega(1)$. 
We will show that there exists $T \in \binom{U}{z - 1}$ that covers all but a constant number of $S \in C$.

Note that we can assume $c \in [0, 1]^U$. Let $c' \in \{ 0, 1 \}^U$ be the {\em rounded vector}; $c'_u = 1$ iff $c_u \geq 0.5$. Let $S'$ be the set indicated by $c'$. 
One crucial observation is that for any $S \in C$, $\| \tau(S) - c \|_2^2 \geq | S \Delta S'|/4$; if $e \in S$ and $e \notin S'$, it means $c_e \leq 0.5$, so $|\tau(S)_e - c_e|^2 \geq 0.25$ (and same for the other case).
It means that $| S \Delta S' | \leq 4$ for all $S \in C$. 

Therefore, we only need to consider the case when $z' := |S'| \in [z-4, z+4]$. 
For each $T \subseteq S'$ create a {\em bucket $B_T$}. For each $S \in C$, put $S$ into $B_{S \cap S'}$. 
Consider a bucket $B_T$ with $|B_T| = \omega(1)$. Such a bucket exists since $|C| = \omega(1)$. 
Let $V := \cup_{S \in B_T} (S \setminus T)$, and consider hypergraph $H = (V, E')$ where
\[
E' := \{ S \setminus T : S \in B_T \}.
\]
Let $r' := z' - |T|$ and $r := z - |T|$ so that $H$ is an $r$-uniform hypergraph. 
Then for each hyperedge $e \in E'$ (that corresponds to $S = e \cup T \in B_T$), 
\begin{align*}
& 1.25 - \eps \geq \| \tau(S) - c \|_2^2 \\
\geq & \sum_{v \in S' \setminus T} (1 - x_v)^2 + \sum_{v \in S \setminus T} (1 - x_v)^2 + \sum_{v \in V \setminus S} x_v^2 \geq 0.25 r' + \sum_{v \in e} (1 - x_v)^2 + \sum_{v \in V \setminus e} x_v^2,
\end{align*}
which is equivalent to
\[
\sum_{v \in e} (1 - x_v)^2 + \sum_{v \in V \setminus e} x_v^2 \leq 1.25 - 0.25r' - \eps = 1 + (1 - r') 0.25 - \eps.
\]
If $1 - r' \leq r - 1$, then Lemma~\ref{lem:hypergraph_l2} shows that $|B_T|$ is bounded by a constant depending on $r$ and $\eps$, contradicting $|B_T| = \omega(1)$. 
Therefore, the only remaining case is $1 - r' > r - 1$, and since both $r', r \geq 0$, we must have $r' = 0$ and $r = 1$. 
This means that $z' = z - 1$ and $S' \subseteq S$ for all $S \in B_T$ whenever $|B_T| = \omega(1)$. 
Since there are at most $2^{z+4}$ buckets, and all but a constant number of sets satisfy $S' \subseteq S$.

Therefore, whenever $|C| = \omega(1)$, in every case, we showed that there exists $S' \in \binom{U}{z - 1}$ that covers all but a constant number of sets in $C$. 
Since $|E| = \omega(k)$, we can use an argument similar to Theorem~\ref{thm:kmeanl2} to show that in the soundness case, the fraction of points that are covered by a center at distance at most $\sqrt{1.25} - \eps$ is at most $(1 - 1/e + \eps)$. Therefore the gap becomes $(1 - 1/e + \eps) + \sqrt{1.25}(1/e - \eps) \approx 1.0434$. 
\end{proof}


We now prove hardness of continuous \kmean in $\ell_1$-metric. We need the following lemma similar to Lemma~\ref{lem:hypergraph_l2}. 

\begin{lemma}\label{lem:hypergraph_l1}
Let $H = (V, E)$ be an $r$-uniform $(r \geq 1)$ hypergraph where each vertex belongs to least one hyperedge, and $x : V \to [0, 0.5]$ such that 
\begin{equation*}
y(e) := \sum_{v \in e} (1 - x_v) + 
\sum_{v \in E \setminus e} x_v \leq 1 + 0.5(r - 1) - \eps \quad \forall e \in E. 
\end{equation*}
for some $\eps > 0$. Then $|E| \leq (2r/\eps + r)^r$. 
\end{lemma}
\begin{proof}
%Since $(1 - x_v) \geq 0.5$, $r$ is either $2$ or $3$.
Suppose that every $v$ satisfies $x_v \geq 2r / (n - r)$. Then for any $e \in E$, 
\[
y(e) \geq \sum_{v \in E \setminus e} x_v \geq (n-r) \frac{2r}{n-r} = 2r,
\]
leading to contradiction. Therefore, there is $v \in V $ that satisfies 
$x_v < 2r / (n - r)$. Choose a hyperedge $e$ containing $v$. Then 
\[
1 - \eps + 0.5(r - 1) \geq y(e) \geq (1 - x_v) + \sum_{u \in e \setminus \{ v \}} x_u \geq (1 - x_v) + 0.5(r - 1) \geq 1 - \frac{2r}{(n - r)} + 0.5(r-1),
\]
which implies 
\[
\eps \leq \frac{2r}{(n - r)} \Leftrightarrow n \leq 2r/\eps + r.
\]
The lemma follows by noting that $|E| \leq n^r$. 
\end{proof}



\begin{theorem}[\kmean without candidate centers in $\poly(n)$-dimensional $\ell_1$-metric space]\label{thm:kmeanl1}
Assuming \JCHD, for every constant $\varepsilon>0$,  given a point-set $\Po\subset \{0,1\}^{d}$ of size $n$ (and $d=\poly(n)$) and a parameter $k$ as input, it is \NP-hard to distinguish between the following two cases:
\begin{itemize}
\item \textbf{\emph{Completeness}}:  
There exists $\C':=\{c_1,\ldots ,c_k\}\subseteq \mathbb \R^d$ and $\sigma:\Po\to\C'$ such that $$\sum_{a\in\Po}\|a-\sigma(a)\|_1^2\le n$$
\item \textbf{\emph{Soundness}}: For every $\C':=\{c_1,\ldots ,c_k\}\subseteq \R^d$ and every $\sigma:\Po\to\C'$ we have: $$\sum_{a\in\Po}\|a-\sigma(a)\|_1^2\ge \left(1+\frac{1.25}{e}-\varepsilon\right)n \approx 1.46n.$$
\end{itemize}
%for some constant $\rho>0$.
\end{theorem}
\begin{proof}
Given an instance $(U, E, k)$ of $(1-1/e+\eps, z)$-\jc for small fixed $\eps > 0$, for any $S \subseteq U$, let $\tau(S)$ be the indicator vector of $S$. In the completeness case, every point is connected to a center at distance $1$.
For the soundness case, fix one cluster $C$ and its center $c \in \R^U$.
Fix $\eps > 0$, and remove all points from $C$ whose $\ell_1$ distance to $c$ is greater than $(1.5 - \eps)$.
Assume $C = \omega(1)$. 
We will show that there exists $T \in \binom{U}{z - 1}$ that covers all but a constant number of $S \in C$.

Note that we can assume $c \in [0, 1]^U$. Let $c' \in \{ 0, 1 \}^U$ be the {\em rounded vector}; $c'_u = 1$ iff $c_u \geq 0.5$. Let $S'$ be the set indicated by $c'$. 
One crucial observation is that for any $S \in C$, $\| \tau(S) - c \|_1 \geq | S \Delta S'|/2$; if $e \in S$ and $e \notin S'$, it means $c_e \leq 0.5$, so $|\tau(S)_e - c_e| \geq 0.5$ (and same for the other case).
It means that $| S \Delta S' | \leq 2$ for all $S \in C$. 

Therefore, we only need to consider the case when $z' := |S'| \in [z-2, z+2]$. 
For each $T \subseteq S'$ create a {\em bucket $B_T$}. For each $S \in C$, put $S$ into $B_{S \cap S'}$. 
Consider a bucket $B_T$ with $|B_T| = \omega(1)$. Such a bucket exists since $|C| = \omega(1)$. 
Let $V := \cup_{S \in B_T} (S \setminus T)$, and consider hypergraph $H = (V, E')$ where
\[
E' := \{ S \setminus T : S \in B_T \}.
\]
Let $r' := z' - |T|$ and $r := z - |T|$ so that $H$ is an $r$-uniform hypergraph. 
Then for each hyperedge $e \in E'$ (that corresponds to $S = e \cup T \in B_T$), 
\begin{align*}
& 1.5 - \eps \geq \| \tau(S) - c \|_1 \\
\geq & \sum_{v \in S' \setminus T} (1 - x_v) + \sum_{v \in S \setminus T} (1 - x_v) + \sum_{v \in V \setminus S} x_v \geq 0.5 r' + \sum_{v \in e} (1 - x_v) + \sum_{v \in V \setminus e} x_v,
\end{align*}
which is equivalent to
\[
\sum_{v \in e} (1 - x_v) + \sum_{v \in V \setminus e} x_v \leq 1.5 - 0.5r' - \eps = 1 + (1 - r') 0.5 - \eps.
\]
If $1 - r' \leq r - 1$, then Lemma~\ref{lem:hypergraph_l1} shows that $|B_T|$ is bounded by a constant depending on $r$ and $\eps$, contradicting $|B_T| = \omega(1)$. 
Therefore, the only remaining case is $1 - r' > r - 1$, and since both $r', r \geq 0$, we must have $r' = 0$ and $r = 1$. 
This means that $z' = z - 1$ and $S' \subseteq S$ for all $S \in B_T$ whenever $|B_T| = \omega(1)$. 
Since there are at most $2^{z+2}$ buckets, and all but a constant number of sets satisfy $S' \subseteq S$.

Therefore, whenever $|C| = \omega(1)$, in every case, we showed that there exists $S' \in \binom{U}{z - 1}$ that covers all but a constant number of sets in $C$. 
Since $|E| = \omega(k)$, we can use an argument similar to Theorem~\ref{thm:kmeanl2} to show that in the soundness case, the fraction of points that are covered by a center at distance at most $1.5 - \eps$ is at most $(1 - 1/e + \eps)$. Therefore the gap becomes $(1 - 1/e + \eps) + 1.5^2(1/e - \eps) = 1 + 1.25 / e - O(\eps) \approx 1.4598$. 
\end{proof}

